Approaching Optimal Duplicate Detection in a Sliding Window

Duplicate detection is the problem of identifying whether a given item has previously appeared in a (possibly infinite) stream of data, when only a limited amount of memory is available. Unfortunately the infinite stream setting is ill-posed, and error rates of duplicate detection filters turn out to be heavily constrained: consequently they appear to provide no advantage, asymptotically, over a biased coin toss [8]. In this paper we formalize the sliding window setting introduced by [13,16], and show that a perfect (zero error) solution can be used up to a maximal window size $w_\text{max}$. Above this threshold we show that some existing duplicate detection filters (designed for the $\textit{non-windowed}$ setting) perform better that those targeting the windowed problem. Finally, we introduce a "queuing construction" that improves on the performance of some duplicate detection filters in the windowed setting. We also analyse the security of our filters in an adversarial setting.

==> er_n_real.tex <==
\nextgroupplot[
	xmode=log,
	xmin = 500,
	xmax = 350000000,
%	extra x ticks = {500},
	xlabel = {Size of the stream},
	ymax = 110,
    ymin = 0,
    ytick = {0, 20, ..., 120},
    ylabel = {FPR + FNR ($\times 100$)},
    title = Real-world data (crawler),
]

%% 1 QHT 
\addplot [color=red, mark=+] coordinates {
	(1000, 0)
	(10000, 0.17)
	(30000, 0.63)
	(50000, 1.22)
	(100000, 2.42)
	(300000, 6.05)
	(1000000, 13.37)
	(3000000, 17.52)
	(10000000, 24.55)
	(50000000, 36.59)
	(100000000, 43.44)
	(150000000, 48.39)
};



%% 2 SQF
\addplot[color=blue, mark=x] coordinates {
	(1000, 0)
	(10000, 0.44)
	(30000, 1.18)
	(50000, 2.2)
	(100000, 4.52)
	(300000, 11.24)
	(1000000, 22.11)
	(3000000, 27.54)
	(10000000, 34.23)
	(50000000, 44.91)
	(100000000, 50.88)
	(150000000, 55.19)
};

%% 3 Cuckoo
\addplot [color=teal, mark=triangle] coordinates {
	(1000, 0.45)
	(10000, 1.85)
	(30000, 6.31)
	(50000, 11.32)
	(100000, 20.9)
	(300000, 37.1)
	(1000000, 47.26)
	(3000000, 50.27)
	(10000000, 54.62)
	(50000000, 61.87)
	(100000000, 66.02)
	(150000000, 68.95)
};

%% 4 SBF 
\addplot [color=olive, mark=square, mark options = {scale=0.7}]coordinates {
	(1000, 0.56)
	(10000, 3.46)
	(30000, 9.04)
	(50000, 13.28)
	(100000, 20.02)
	(300000, 27.19)
	(1000000, 31.97)
	(3000000, 32.86)
	(10000000, 37.76)
	(50000000, 47.48)
	(100000000, 53.13)
	(150000000, 57.18)
};

%%% 5 A2 
%\addplot [color=orange, mark=diamond]coordinates {
%	(1000, 0)
%	(10000, 0.07)
%	(30000, 0.36)
%	(50000, 0.86)
%	(100000, 3.33)
%	(300000, 17.72)
%	(1000000, 33.66)
%	(3000000, 38.6)
%	(10000000, 44.43)
%	(50000000, 53.47)
%	(100000000, 58.52)
%	(150000000, 62.15)
%};

\coordinate (top) at (rel axis cs:0,1);
\coordinate (bot) at (rel axis cs:1,0);
%%% 5 bDBF 
%\addplot [color=magenta, mark=pentagon]coordinates {
%	(1000, 0.11)
%	(10000, 0.07)
%	(30000, 0.35)
%	(50000, 2.44)
%	(100000, 7.18)
%	(300000, 10.43)
%	(1000000, 14.39)
%	(3000000, 14.85)
%	(10000000, 20.72)
%	(50000000, 33.02)
%	(100000000, 40.15)
%	(150000000, 45.32)
%};

==> graphs/bench_shorts.tex <==
\begin{tikzpicture}
\begin{semilogxaxis}[%legend pos = outer north east, 
	legend style={at={(0.02,0.98)},anchor=north west},%
	xlabel=$w$, ylabel=$\FPR^w+\FNR^w (\times 100)$]

\addplot[color=blue, mark=o] table[x=w,y=Error] {graphs/shf.dat};
\addlegendentry{SHF}

%\addplot[color=red, mark=x] table[x=a,y=b] {graphs/CSHF.dat};
%\addlegendentry{CSHF}

\end{semilogxaxis}
\end{tikzpicture}

